Constructing Variables Using Classifiers as an Aid to Regression: An Empirical Assessment

This paper proposes a method for the automatic creation of variables (in the case of regression) that complement the information contained in the initial input vector. The method works as a pre-processing step in which the continuous values of the variable to be regressed are discretized into a set of intervals which are then used to define value thresholds. Then classifiers are trained to predict whether the value to be regressed is less than or equal to each of these thresholds. The different outputs of the classifiers are then concatenated in the form of an additional vector of variables that enriches the initial vector of the regression problem. The implemented system can thus be considered as a generic pre-processing tool. We tested the proposed enrichment method with 5 types of regressors and evaluated it in 33 regression datasets. Our experimental results confirm the interest of the approach.

==> annexe.tex <==
\section*{Annexe}

\subsection*{A-1 : Illustration de la définition des seuils}


La figure \ref{fig:seuils} illustre l'étape qui consiste à définir des seuils ($S$) sur l'espace de la variable à régresser.

\begin{figure}[h]
	\begin{center}
		\includegraphics[width=0.45\textwidth]{illustrations/seuils_sur_y.png}
		\caption{Exemple de seuils}
		\label{fig:seuils}
	\end{center}
%\vspace{-4mm}
\end{figure}

\subsection*{A-2 : Illustration de l'extension du vecteur $X$}

La figure \ref{fig:DatasetExtension} illustre l'extension du vecteur $X$ (ayant $d$ composantes) au vecteur $X''$ (ayant $d+S$ composantes). 

\begin{figure}[h]
	\begin{center}
		\includegraphics[width=0.75\textwidth]{illustrations/dataset_etendu.png}
		\caption{Extension de l'ensemble de données.}
		\label{fig:DatasetExtension}
	\end{center}
%\vspace{-4mm}
\end{figure}

\subsection*{A-3 : Schématisation du principe général de la méthode}

La figure \ref{fig:generalprinciple} résume le processus suivi par la méthode proposée.

\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.75\textwidth]{illustrations/principe_general.png}
		\caption{Schématisation du principe général de la méthode.}
		\label{fig:generalprinciple}
	\end{center}
%\vspace{-4mm}
\end{figure}

\subsection*{A-4 : Détails suppleméntaires sur les variables extraites ($X'$)}

Pour la phase expérimentale qui a été mise en place, les variables extraites par la méthode proposée sont les probabilités conditionnelles prédites par chaque classifieur. Plus précisément, chaque classifieur a été entraîné à prédire si les données que l'on lui fournit sont inférieures ou supérieures au seuil auquel il est associé. Les probabilités conditionnelles de la classe 1 (c'est a dire si $y \geq y_i$) prédites par chaque classifieur composeront donc le vecteur $X'=\{X'_1, ..., X'_i, ..., X'_S\}$ (avec $S$ le nombre de seuils) qui sera ajouté à l'ensemble de données initial.

Pour pouvoir extraire cette probabilité conditionnelle, il faut donc un classifieur capable de générer ce genre de résultats. Dans le cas des forêts aléatoires qui ont été utilisées comme modèle de classification au sein de notre méthode pour les résultats présentés dans cet article, la probabilité conditionnelle correspond à la proportion d'arbres ayant voté pour une certaine classe. Avec 100 arbres dans les forêts qui ont été définies, la précision de la prédiction sera donc à 0.01 près.


\subsection*{A-5 : Détails sur les jeux de données et prétraitements}
\label{datasets}

\begin{table*}[!h]
    \centering
    % ci-dessous deux commandes magiques pour que le tableau entre dans la largeur de la page ;-)
    \fontsize{7}{9}\selectfont
    \setlength{\tabcolsep}{2pt}
    % \setlength{\tab}{2pt}    % => undefined control sequence lorsqu'on l'inclut
    \begin{tabular}{|l|l|l|l||l|l|l|l|}
        \hline
        Jeu de données       & \#individus    & \# variables & target & Jeu de données       & \#individus    & \# variables & target\\ \hline
        \hline
        3Droad               & 434,874        & 3       & altitude   & geo-lat              & 1,059          & 116     & latitude\\ \hline
        air-quality-CO       & 1,230          & 8       & PT08.S1(CO)  & greenhouse-net       & 955,167        & 15      & synthetic var  \\ \hline
        airfoil              & 1,503          & 5       & scaled sound  & KEGG-reaction        & 65,554         & 27      & edge count\\ \hline
        appliances-energy    & 19,735         & 26      & appliances    &   KEGG-relation        & 54,413         & 22      & clustering coef  \\ \hline
        beijing-pm25         & 41,758         & 14      & PM2.5 & online-news          & 39,644         & 59      & shares \\ \hline
        temp-forecast-bias   & 7,752          & 22      & Next\_Tmax &  video-transcode      & 68,784         & 26      & utime\\ \hline
        bike-hour            & 17,379         & 17      & count  &  pm25-chengdu-us      & 27,368         & 20      & PM\_US Post\\ \hline
        blog-feedback        & 60,021         & 18      & target  &  park-total-UPDRS     & 5,875          & 16      & total\_UPDRS\\ \hline
        buzz-twitter         & 583,250        & 70      & discussions &  physico-protein      & 45,730         & 9       & RMSD \\ \hline
        combined-cycle       & 9,568          & 4       & PE   & production-quality   & 29,184         & 17      & quality \\ \hline
        com-crime            & 1,994          & 122     & Violent crimes &  CT-slices            & 53,500         & 384     & reference  \\ \hline
        com-crime-unnorm     & 2,215          & 134     & Violent crimes  & gpu-kernel-perf      & 241,600        & 14      & Run1 (ms) \\ \hline
        compress-stren       & 1,030          & 8       & compressive strength & SML2010              & 4,137          & 26      & indoor temp \\ \hline
        cond-turbine         & 11,934         & 15      & gt turbine & seoul-bike-sharing   & 8,760          & 9      & Rented Bike Count  \\ \hline
        cuff-less            & 61,000         & 2       & APB  & uber-location-price  & 205,670        & 5       & fare amount\\ \hline
        electrical-grid-stab & 10,000         & 12      & stab  &  year-prediction      & 515,345        & 90      & Year \\ \hline
        facebook-comment     & 40,949         & 53      & target & & & & \\ \hline
	\end{tabular}
    \caption{Description des 33 jeux de données. La première colonne  désigne le nom du jeu (ou du sous-jeu) de données provenant de l'UCI ou de Kaggle.  La deuxième et la troisième colonne donnent respectivement le nombre d'individus  et le nombre de variables (explicatives) initial du jeu de données (après les étapes de prétraitements). Enfin la quatrième colonne indique le nom de la variable cible à régresser.}
	\label{table:DatasetsDescription}
\end{table*}


Pour réaliser l'analyse de la méthode proposée, nous avons sélectionné une large collection de jeux de données de régression provenant du UCI Repository \citep{Dua:2019} ou de Kaggle. %\citep{kaggle}. 
Au total, 33 jeux de données ont été utilisés, parmi lesquels 23 sont constitués de plus de 10 000 individus. Les 10 jeux de données restants  allant de 1 030 à 9 568 individus (voir Table \ref{table:DatasetsDescription}). Certains de ces jeux de données comprenaient plusieurs sous-ensembles de données avec différentes variables cibles à régresser, et donc différents problèmes de régression. Il a été choisi de ne pas inclure  plusieurs problèmes de régression provenant des mêmes ensembles de données, afin de pas donner plus de poids à certains ensembles de données et créer un biais dans la comparaison des méthodes qui pourrait favoriser une méthode par rapport à une autre. Le lecteur pourra se référer à la colonne "nom de l'ensemble de données" de la Table \ref{table:DatasetsDescription} qui désigne le problème de régression utilisé pour chaque jeu de données.




\subsection*{A-6 : Détails supplémentaires sur les régresseurs utilisés}

Lors des expérimentations, cinq régresseurs utilisant des cadres différents ont été utilisés. Ils sont cités dans l'article. Il sont davantage décrits  ci-dessous, tout en étant largement connus par la communauté de l'apprentissage automatique.

{$\bullet$ Régression Linéaire (LR\footnote{Dans la suite les acronymes anglais seront utilisés.}) : }
La régression désigne le processus d'estimation d'une variable numérique continue à l'aide d'autres variables qui lui sont corrélées. Cela signifie que les modèles de régression prennent la forme de $y=f(X)$ où $y$ peut prendre un ensemble infini de valeurs. Dans cet article, nous avons choisis une régression linéaire multivariée dont le modèle, $f$, est déterminé par la méthode des moindres carrés. Nous avons utilisé la version 0.24.2 de Scikit-Learn. 
Ce modèle ne nécessite pas d'optimisation de ses paramètres.

%\textcolor{blue}{VL: en dehors de la version se scikit learn il faut aussi indiquer : quelle version de RL a été utilisée, idem ci-dessous pour l'arbre, RF , XGboost (s'il en existe plusieurs dans ScikitLearn) )} 


{$\bullet$ Arbre de Régression (DT) : }
Les arbres de décision permettent de prédire une quantité réelle qui, dans le cas de régression, est une valeur numérique. Usuellement, les algorithmes pour construire les arbres de décision sont construits en divisant l'arbre du sommet vers les feuilles en choisissant à chaque étape une variable d'entrée qui réalise le meilleur partage de l'ensemble d'objets. 
Dans le cas des arbres de régression, on cherche à maximiser la variance inter-classes (avoir des sous-ensembles dont les valeurs de la variable-cible sont le plus dispersées possibles). Dans cet article, nous avons utilisé la version 0.24.2 de Scikit-Learn. Ce modèle  nécessite une optimisation de ses paramètres.

{$\bullet$ Forêt aléatoire (RF) : } Les forêts d'arbres décisionnels (ou forêts aléatoires de l'anglais Random Forest (RF) régresseur) ont été  proposées par Ho en 1995 %\citep{RandomDecisionForests} 
[Ho, T. K. (1995). Random decision forests. In Proceedings of 3rd International Conference
on Document Analysis and Recognition, Volume 1, pp. 278–282 vol.1.]
puis étendu par Leo Breiman et Adele Cutler [Breiman, L. (2001). Random forests. Machine Learning 45, 5–32.]
%\citep{RandomForestsBreiman}. 
Cet algorithme combine les concepts de sous-espaces aléatoires et de bagging. L'algorithme des forêts d'arbres décisionnels effectue un apprentissage sur de multiples arbres de décision entraînés sur des sous-ensembles de données légèrement différents. Dans cet article, nous avons utilisé la version 0.24.2 de Scikit-Learn. Ce modèle  nécessite une optimisation de ses paramètres.

{$\bullet$ XGBoost (XGB): }
XGBoost [Chen, T. et C. Guestrin (2016). Xgboost : A scalable tree boosting system. In the 22nd ACM
SIGKDD International Conference, pp. 785–794.]
%\citep{xgboostpaper}
est une méthode de boosting. Elle combine séquentiellement des apprenants faibles qui  présenteraient individuellement de mauvaises performances pour améliorer la prédiction de l'algorithme complet. Un apprenant faible est un régresseur qui a une faible performance de régression. Dans cet algorithme de boosting, des poids élevés seront associés aux apprenants faibles ayant une bonne précision, et à l'inverse, des poids plus faibles aux apprenants faibles ayant une mauvaise précision. Dans la phase d'entraînement, des poids élevés sont associés aux données qui ont été mal "apprises" afin que l'apprenant faible suivant dans la séquence se concentre davantage sur ces données. Dans cet article, nous avons utilisé la version 1.4.1 de XGBoost. Ce modèle  nécessite une optimisation de ses paramètres.

{$\bullet$  Na\"ive Bayes Pondéré (SNB): }
Dans le contexte de la régression, un régresseur naïf de Bayes (NB) dont les variables sont pondérées par des poids (NBP) peut être obtenu à l'aide de deux étapes.
Dans un premier temps, pour chaque variable explicative, on crée une grille 2D pour estimer $P(X,y)$ (voir par exemple [Boullé, M. (2006). MODL : a Bayes optimal discretization method for continuous attributes. Machine Learning 65(1), 131–165.])
%(voir par exemple \citep{MODLBoulleML06}). 
Ensuite, dans une deuxième étape, toutes les variables sont regroupées dans un algorithme Forward Backward 
%\citep{BoulleJMLR07}
pour estimer leur informativité dans le contexte d'un régresseur Naïf de  Bayes. A la fin de la deuxième étape, le modèle final (à déployer) est un Na\"ive Bayes (qui utilise la discrétisation 2D trouvée dans la première étape) où les variables sont pondérées (les poids sont trouvés dans la deuxième étape). Dans cet article nous avons utilisé le Na\"ive Bayes Pondéré produit par le logiciel Khiops  ({\url{www.khiops.com}}). Nous avons demandé et obtenu gratuitement une licence provisoire du logiciel  ainsi que sa version pyKhiops utilisable dans Scikit-Learn. Ce modèle ne nécessite pas d'optimisation de ses paramètres.





